Attractor scenarios and superluminal signals in k-essence cosmology

Cosmological scenarios with k-essence are invoked in order to explain the observed late-time acceleration of the universe. These scenarios avoid the need for fine-tuned initial conditions (the "coincidence problem") because of the attractor-like dynamics of the k-essence field \phi. It was recently shown that all k-essence scenarios with Lagrangians p=L(X)/\phi^2, necessarily involve an epoch where perturbations of \phi propagate faster than light (the "no-go theorem"). We carry out a comprehensive study of attractor-like cosmological solutions ("trackers") involving a k-essence scalar field \phi and another matter component. The result of this study is a complete classification of k-essence Lagrangians that admit asymptotically stable tracking solutions, among all Lagrangians of the form p=K(\phi)L(X) . Using this classification, we select the class of models that describe the late-time acceleration and avoid the coincidence problem through the tracking mechanism. An analogous "no-go theorem" still holds for this class of models, indicating the existence of a superluminal epoch. In the context of k-essence cosmology, the superluminal epoch does not lead to causality violations. We discuss the implications of superluminal signal propagation for possible causality violations in Lorentz-invariant field theories.

==> ket1a.tex <==

\section{Transient attractor solutions\label{sec:Stable-transient-solutions}}

In typical scenarios of $k$-essence, there is an epoch when the $k$-essence
has negligible energy density compared with the matter component. The solution
of the dynamical equations during this epoch is also an attractor for nearby
solutions. Eventually the energy density of the $k$-essence starts to dominate
and this epoch ends, giving place to another attractor solution. We may call
this temporary attractor solution a {}``transient'' attractor. The attractor
nature of the solution is needed to avoid the fine-tuning of initial conditions
for the timely onset of the $k$-essence domination epoch. We will now investigate
the existence of transient attractor solutions.

The mathematical technique we will use to study the transient attractor solution
is the following. We will modify the basic equations of motion~(\ref{eq:v equ})--(\ref{eq:epsilon m equ}),
replacing $\varepsilon_{\text{tot}}$ by $\varepsilon_{m}$. This yields the
equations \begin{align}
\frac{dv(\phi)}{d\phi} & =-\frac{vp_{,v\phi}-p_{,\phi}+3\kappa p_{,v}\sqrt{\varepsilon_{m}}}{vp_{,vv}},\label{eq:v equ 14}\\
\frac{d\varepsilon_{m}}{d\phi} & =-\frac{3\kappa\left(1+w_{m}\right)\varepsilon_{m}}{v}\sqrt{\varepsilon_{m}}.\label{eq:epsilon m equ 14}\end{align}
Solutions of these equations will approximately coincide with the correct solutions
as long as $\varepsilon_{\phi}\ll\varepsilon_{m}$. By the usual techniques
of asymptotic analysis, we will search for solutions of Eqs.~(\ref{eq:v equ 14})--(\ref{eq:epsilon m equ 14})
that exhibit a stable asymptotic behavior at $\phi\rightarrow\infty$ and a
significant growth of the ratio $\varepsilon_{\phi}/\varepsilon_{m}$. These
solutions, if found, will be interpreted as transient attractors. The growth
of $\varepsilon_{\phi}/\varepsilon_{m}$ requires that $w_{\phi}<w_{m}$ at
all times; however, the case $w_{\phi}(\phi)\rightarrow w_{m}$ as $\phi\rightarrow\infty$
is not excluded a priori.

It is convenient to introduce an auxiliary variable\begin{equation}
h\equiv\frac{1}{3\kappa\sqrt{\varepsilon_{m}}},\label{eq:h def 15}\end{equation}
and to rewrite Eqs.~(\ref{eq:v equ 14})--(\ref{eq:epsilon m equ 14}) for
the Lagrangian~(\ref{eq:Kessence L2}) as\begin{align}
\frac{dv}{d\phi} & =-c_{s}^{2}(v)\left(\frac{v}{1+w_{\phi}(v)}\frac{K'}{K}+\frac{1}{h}\right),\label{eq:v equ 15}\\
\frac{dh}{d\phi} & =\frac{1+w_{m}}{2v}.\label{eq:h equ 15}\end{align}
It is clear that the behavior of the solutions depends on whether $v\rightarrow0$,
$c_{s}^{2}\rightarrow0$, or $1+w_{\phi}(v)\rightarrow0$ at large $\phi$.
This is determined by the function $Q(v)$ and by the asymptotic value $v_{0}\equiv\lim_{\phi\rightarrow\infty}v(\phi)$.
Therefore we consider the cases $v_{0}=0$ and $v_{0}\neq0$ separately.

In case $v_{0}\neq0$, it follows from Eq.~(\ref{eq:epsilon m equ 14}) that
the asymptotic behavior of $\varepsilon_{m}(\phi)$ is $\varepsilon_{m}\propto\phi^{-2}$
at large $\phi$. We begin by considering this case.

The function $Q(v)$ near $v=v_{0}$ has a Taylor expansion of the form\begin{equation}
Q(v)=Q(v_{0})+\left(v-v_{0}\right)Q'(v_{0})+\frac{1}{2}\left(v-v_{0}\right)^{2}Q^{\prime\prime}(v_{0})+...,\end{equation}
where the coefficients $Q(v_{0})$ and $Q'(v_{0})$ are nonzero for a generic
value of $v_{0}$ (moreover, $Q'(v_{0})>0$ due to the considerations of Sec.~\ref{sec:Physical restrictions}).
It follows that \begin{align}
w_{\phi}(v_{0}) & =\frac{Q(v_{0})}{v_{0}Q'(v_{0})-Q(v_{0})}>-1,\label{eq:wk cond 15 positive}\\
c_{s}^{2}(v_{0}) & =\frac{Q'(v_{0})}{v_{0}Q^{\prime\prime}(v_{0})}\neq0.\end{align}
 Finiteness of $c_{s}^{2}(v_{0})$ requires also $Q^{\prime\prime}(v_{0})\neq0$.
This is the generic case studied in Sec.~\ref{sub:Energy-density-transient-1}. 

If $v_{0}$ is such that $Q'(v_{0})=0$, then Eq.~(\ref{eq:Q expansion Q0})
applies, and assuming that $Q(v_{0})\neq0$, we may use the expansions for $c_{s}^{2}(v)$
and $w_{\phi}(v)$ given in Eqs.~(\ref{eq:wk expansion Q0})--(\ref{eq:cs expansion Q0}).
There remain the possibilities $Q(v_{0})=0$ and $Q'(v_{0})>0$ (note that $Q'(v_{0})<0$
is excluded by the considerations of Sec.~\ref{sec:Physical restrictions}),
or $Q(v_{0})=0$ and $Q'(v_{0})=0$. All these possibilities will be considered
below.

Let us begin by deriving some results that hold in all cases when $v_{0}\neq0$.
Taking the limit of Eq.~(\ref{eq:v equ 15}) as $\phi\rightarrow\infty$, we
obtain\begin{equation}
\lim_{\phi\rightarrow\infty}h'(\phi)=\frac{1+w_{m}}{2v_{0}}\equiv h_{0}.\label{eq:h0 def 15}\end{equation}
It follows that \begin{equation}
\lim_{\phi\rightarrow\infty}\frac{d}{d\phi}\left(h(\phi)-h_{0}\phi\right)=0,\end{equation}
so the function $h-h_{0}\phi$ grows slower than $\propto\phi$ at $\phi\rightarrow\infty$.
Therefore we may use the ansatz\begin{equation}
h(\phi)=h_{0}\phi\left[1+C(\phi)\right],\quad v(\phi)=v_{0}+A(\phi),\label{eq:ansatz 15}\end{equation}
where the unknown functions $A(\phi)$ and $C(\phi)$ tend to zero at $\phi\rightarrow\infty$.
Substituting this ansatz into Eqs.~(\ref{eq:v equ 15})--(\ref{eq:h equ 15}),
we find \begin{align}
\frac{dA}{d\ln\phi} & =-c_{s}^{2}(v)\left(\frac{v}{1+w_{\phi}(v)}\frac{d\ln K}{d\ln\phi}+\frac{1}{h_{0}\left(1+C\right)}\right).\label{eq:A equ 15a}\\
\frac{dC}{d\ln\phi} & =-\frac{1}{v_{0}}A-C.\label{eq:h equ 15a}\end{align}
In some cases (to be found below) when Eq.~(\ref{eq:A equ 15a}) is independent
of $C(\phi)$ in the leading order, Eq.~(\ref{eq:h equ 15a}) shows that the
solution $C(\phi)$ tends to zero as long as $A(\phi)$ tends to zero.


\subsection{Energy density $\varepsilon_{m}\propto\phi^{-2}$, main case\label{sub:Energy-density-transient-1}}

In this section we consider the generic case $v_{0}\neq0$, $c_{s}^{2}(v_{0})\neq0$,
$w_{\phi}(v_{0})\neq-1$, which is found when $Q(v_{0})\neq0$, $Q'(v_{0})\neq0$.
Taking the limit of Eq.~(\ref{eq:A equ 15a}) at $\phi\rightarrow\infty$ gives
for stable solutions the necessary condition\begin{equation}
\frac{v_{0}}{1+w_{\phi}(v_{0})}\lim_{\phi\rightarrow\infty}\frac{d\ln K}{d\ln\phi}+\frac{1}{h_{0}}=0.\end{equation}
 It follows that\begin{equation}
2\frac{1+w_{\phi}(v_{0})}{1+w_{m}}=-\lim_{\phi\rightarrow\infty}\frac{d\ln K}{d\ln\phi}\equiv2\alpha,\label{eq:v0 equ 15}\end{equation}
where we must have \begin{equation}
0<\alpha\leq1\end{equation}
since $w_{\phi}(v_{0})>-1$ due to Eq.~(\ref{eq:wk cond 15 positive}), while
$w_{\phi}(v_{0})\leq w_{m}$ by assumption. The limit~(\ref{eq:v0 equ 15})
exists when $K(\phi)$ is of the form\begin{equation}
K(\phi)=\phi^{-2\alpha}K_{0}(\phi),\quad\lim_{\phi\rightarrow\infty}\frac{d\ln K_{0}}{d\ln\phi}=0,\label{eq:K ansatz 15}\end{equation}
where the function $K_{0}(\phi)$ may be arbitrary as long as it grows (or decays)
slower than any power of $\phi$. For a given Lagrangian with $K(\phi)$ of
this form, the value of $\alpha$ is known and then the possible values of $v_{0}$
are determined by Eq.~(\ref{eq:v0 equ 15}).

For $K(\phi)$ of the form given above, we may linearize Eq.~(\ref{eq:A equ 15a})
with the ansatz~(\ref{eq:ansatz 15}), (\ref{eq:K ansatz 15}). After some
algebra using Eq.~(\ref{eq:derivative of wk}), we obtain\begin{align}
\frac{dA}{d\ln\phi} & =\frac{2w_{\phi}(v_{0})}{1+w_{m}}A+\frac{2v_{0}c_{s}^{2}(v_{0})}{1+w_{m}}C-\frac{c_{s}^{2}(v_{0})v_{0}}{1+w_{\phi}(v_{0})}\frac{d\ln K_{0}}{d\ln\phi}.\label{eq:v equ 15a}\end{align}
The system~(\ref{eq:h equ 15a}), (\ref{eq:v equ 15a}) is of the form~(\ref{eq:A hom equ})--(\ref{eq:C hom equ})
with an additional inhomogeneous term, which tends to zero at $\phi\rightarrow\infty$.
According to the stability criterion derived in Sec.~\ref{sub:Energy-density-dominates-1},
solutions of the inhomogeneous system are asymptotically stable if both the
eigenvalues of the homogeneous system have negative real parts. The corresponding
conditions are found to be\begin{equation}
w_{\phi}(v_{0})<\frac{1+w_{m}}{2},\quad c_{s}^{2}(v_{0})>w_{\phi}(v_{0}).\end{equation}
Expressing $w_{\phi}(v_{0})$ through $\alpha$ from Eq.~(\ref{eq:v0 equ 15}),
we transform the first of these inequalities to\begin{equation}
\alpha<\frac{1}{2}+\frac{1}{1+w_{m}}.\end{equation}
When $w_{m}<1$, the inequality above is weaker than the earlier assumption
$\alpha\leq1$ and can be omitted. 

We can now exclude the possibility $\alpha=1$ (equivalently, $w_{\phi}(v_{0})=w_{m}$)
by requiring that the ratio $\varepsilon_{\phi}/\varepsilon_{m}$ grows at least
to order 1. The quantity $R\equiv\varepsilon_{m}/\varepsilon_{\text{tot}}$
should reach at least $\frac{1}{2}$, while initially $R\approx1$. If $w_{\phi}(v_{0})=w_{m}$,
we use the ansatz~(\ref{eq:ansatz 15}) to get\begin{equation}
w_{m}-w_{\phi}(v)=-w_{\phi}^{\prime}(v_{0})A,\end{equation}
and then we rewrite Eq.~(\ref{eq:R equ 0}) to the leading order, substituting
$H=\kappa\sqrt{\varepsilon_{m}}=1/(3h)$, as\begin{equation}
\frac{dR}{d\ln\phi}=\frac{1}{h_{0}v_{0}}R(1-R)w_{\phi}^{\prime}(v_{0})A.\end{equation}
Since the general solution $A(\phi)$ tends to zero as a power of $\phi$, e.g.\begin{equation}
A(\phi)=A_{0}\left(\frac{\phi}{\phi_{0}}\right)^{-\lambda},\quad\lambda>0,\end{equation}
the general solution $R(\phi)$ will tend to a constant which depends on the
initial value $A_{0}\equiv A(\phi_{0})$. For a very small $A_{0}$, the value
of $R$ can be approximated as\begin{equation}
R(\phi)\approx R_{0}-\frac{R_{0}(1-R_{0})}{h_{0}v_{0}}w_{\phi}^{\prime}(v_{0})\frac{A_{0}}{\lambda}\left[\left(\frac{\phi}{\phi_{0}}\right)^{-\lambda}-1\right],\end{equation}
where $R_{0}$ is the initial value of $R(\phi)$. Thus $R(\phi)$ will change
by a very small amount as $\phi\rightarrow\infty$ and will not reach $\frac{1}{2}$.
Therefore, the case $w_{\phi}(v_{0})=w_{m}$ does not admit a transient attractor
solution.

Thus the general solution is stable if $K(\phi)$ is of the form~(\ref{eq:K ansatz 15})
with $0<\alpha<1$ and $c_{s}^{2}(v_{0})>w_{\phi}(v_{0})$, where $v_{0}$ is
determined by Eq.~(\ref{eq:v0 equ 15}), and if the assumptions $Q(v_{0})\neq0$,
$Q'(v_{0})\neq0$ hold. In the next subsections we relax these two latter assumptions.


\subsection{Energy density $\varepsilon_{m}\propto\phi^{-2}$, de Sitter attractor}

In this section we consider the case $Q(v_{0})\neq0$, $Q'(v_{0})=0$, which
leads to the expansions~(\ref{eq:Q expansion Q0})--(\ref{eq:cs expansion Q0})
with $n\geq2$. (The condition $Q'(v_{0})=0$ determines the possible values
of $v_{0}$, and we have $w_{\phi}(v_{0})=-1$.) Using these expansions and
the ansatz~(\ref{eq:ansatz 15}), we rewrite Eq.~(\ref{eq:A equ 15a}) in
the leading order as\begin{equation}
\frac{d}{d\ln\phi}A^{n-1}=\frac{Q_{0}}{v_{0}}\frac{1+O(A)}{nQ_{1}}\frac{d\ln K}{d\ln\phi}-\frac{1+O(C)}{v_{0}h_{0}}A^{n-1}.\label{eq:A equ 15b}\end{equation}
Taking the limit of this equation at $\phi\rightarrow\infty$, we obtain the
necessary condition for a stable solution,\begin{equation}
\lim_{\phi\rightarrow\infty}\frac{d\ln K}{d\ln\phi}=0.\label{eq:K cond 15b}\end{equation}
Under this assumption, the terms $O(A)$ and $O(C)$ can be omitted from Eq.~(\ref{eq:A equ 15b})
for the purposes of stability analysis. Since $h_{0}>0$ and $v_{0}>0$, we
find that the solution $A(\phi)$ always tends to zero under the condition~(\ref{eq:K cond 15b}).
The solution $C(\phi)$ also tends to zero when $A(\phi)\rightarrow0$, as can
be seen from Eq.~(\ref{eq:h equ 15a}). Thus the condition~(\ref{eq:K cond 15b})
is also sufficient for the asymptotic stability of the general solution. This
solution is a transient attractor because $w_{\phi}(v_{0})=-1<w_{m}$.


\subsection{Energy density $\varepsilon_{m}\propto\phi^{-2}$, dust attractor ($w_{\phi}(v_{0})=0$)}

Dust attractor solutions may be possible in case $Q(v_{0})=0$, which fixed
the possible values of $v_{0}$. If (generically) $Q'(v_{0})>0$, we have the
following expansions at large $\phi$:\begin{align}
Q(v) & \approx Q_{1}(v-v_{0})+Q_{2}\left(v-v_{0}\right)^{n},\quad n\geq2,\quad Q_{1}>0;\\
w_{\phi}(v) & \approx\frac{v-v_{0}}{v_{0}},\\
c_{s}^{2} & \approx\frac{Q_{1}}{v_{0}n(n-1)Q_{2}(v-v_{0})^{n-2}}.\end{align}
Reasonable values of the speed of sound, $0<c_{s}^{2}<\infty$, can be obtained
only if $n=2$ and $Q_{2}>0$. Since in that case $w_{\phi}(v_{0})\neq-1$ and
$c_{s}^{2}(v_{0})\neq0$, the conclusions of Sec.~\ref{sub:Energy-density-transient-1}
fully apply to the present case, with the additional constraint $w_{\phi}(v_{0})=0$.
Thus, a transient attractor solution exists only for $K(\phi)$ of the form\begin{equation}
K(\phi)\propto\phi^{-2\alpha}K_{0}(\phi),\quad\lim_{\phi\rightarrow\infty}\frac{d\ln K_{0}(\phi)}{d\ln\phi}=0,\end{equation}
where\begin{equation}
\alpha=\frac{1}{1+w_{m}},\quad w_{m}>0.\end{equation}


It remains to consider the marginal case $Q(v_{0})=0$ and $Q'(v_{0})=0$. In
that case we have the following expansions at large $\phi$,\begin{align}
Q(v) & \approx Q_{1}\left(v-v_{0}\right)^{n},\quad n\geq2,\quad Q_{1}>0,\\
w_{\phi}(v) & \approx\frac{v-v_{0}}{nv_{0}},\label{eq:wk expansion 16}\\
c_{s}^{2} & \approx\frac{v-v_{0}}{v_{0}(n-1)}.\end{align}
Using these expansions, the ansatz~(\ref{eq:ansatz 15}), and the definition~(\ref{eq:h0 def 15})
of $h_{0}$, we can linearize Eq.~(\ref{eq:A equ 15a}) as\begin{equation}
\frac{dA}{d\ln\phi}=-\frac{A}{n-1}\left(\frac{d\ln K}{d\ln\phi}+\frac{2}{1+w_{m}}\right),\end{equation}
which can be integrated and yields\begin{equation}
A(\phi)=C_{0}\left[K(\phi)\phi^{\frac{2}{1+w_{m}}}\right]^{-\frac{1}{n-1}},\end{equation}
where $C_{0}>0$ is an integration constant. Hence, the general solution for
$A(\phi)$ will tend to zero if $K(\phi)$ is such that\begin{equation}
\lim_{\phi\rightarrow\infty}K(\phi)\phi^{\frac{2}{1+w_{m}}}=\infty.\end{equation}
Under this condition, the general solution for $C(\phi)$ will also tend to
zero due to Eq.~(\ref{eq:h equ 15a}). Thus, the presently considered solution
is an attractor.

Finally, we need to investigate whether this attractor is transient. The condition
$w_{m}>0$ is sufficient, while the possibility $w_{m}=0$ is excluded: According
to the expansion~(\ref{eq:wk expansion 16}), we have $w_{\phi}(v)>0$ at all
times, and so the energy density of $k$-essence cannot become dominant if $w_{m}=0$.
We conclude that $w_{m}>0$ is both sufficient and necessary for the presently
considered attractor to be transient.


\subsection{Slow motion ($v_{0}=0$), de Sitter attractor}

We now consider the case $v_{0}=0$. Similarly to the analysis in Sec.~\ref{sub:Slow-motion-main-case},
we deduce that $Q'(0)=0$. Then $Q(v)$ has the expansion~(\ref{eq:Q expansion 3}),
and we need to distinguish the cases $Q(0)\neq0$ and $Q(0)=0$. If $Q(0)\neq0$,
we can use the expansions~(\ref{eq:wk expansion 3})--(\ref{eq:cs expansion 3}).
For $Q(0)=0$ we need to use Eq.~(\ref{eq:wk expansion 3a}) as the expansion
for $w_{\phi}(v)$, while Eq.~(\ref{eq:cs expansion 3}) still applies.

In this section we consider the generic case $Q(0)\neq0$. According to Eq.~(\ref{eq:wk expansion 3}),
we then have $w_{\phi}(0)=-1$, indicating a possible de Sitter attractor. Using
the expansions~(\ref{eq:wk expansion 3})--(\ref{eq:cs expansion 3}), we rewrite
Eqs.~(\ref{eq:v equ 15})--(\ref{eq:h equ 15}) to leading order as\begin{align}
\frac{dv^{n}}{d\phi} & =-\frac{1}{n-1}\frac{Q_{0}}{Q_{1}}\frac{K'}{K}-\frac{n}{n-1}v^{n-1}h^{-1},\label{eq:v equ 17}\\
\frac{dh}{d\phi} & =\frac{1+w_{m}}{2}v^{-1}.\label{eq:h equ 17}\end{align}
For solutions with $v(\phi)\rightarrow0$ we must have $h(\phi)\rightarrow\infty$
faster than $\phi$, i.e.~$\lim_{\phi\rightarrow\infty}\phi^{-1}h=\infty$.
Therefore it is convenient to introduce an auxiliary function \begin{equation}
f(\phi)\equiv\frac{2}{1+w_{m}}\frac{h(\phi)}{\phi},\quad\lim_{\phi\rightarrow\infty}f(\phi)=\infty,\end{equation}
change the variable $\phi\rightarrow\psi$,\begin{equation}
\psi\equiv\frac{2}{\left(1+w_{m}\right)\left(n-1\right)}\ln\phi,\end{equation}
and to rewrite Eqs.~(\ref{eq:v equ 17})--(\ref{eq:h equ 17}) as\begin{align}
\frac{dv}{d\psi} & =-\frac{Q_{2}}{v^{n-1}}\left(\ln K\right)_{,\psi}-\frac{1}{f},\quad Q_{2}\equiv\frac{1}{n\left(n-1\right)}\frac{Q_{0}}{Q_{1}}>0,\label{eq:v equ 17a}\\
\frac{d\ln f}{d\psi} & =\left(\frac{1}{fv}-1\right)\frac{\left(n-1\right)\left(1+w_{m}\right)}{2}.\label{eq:f equ 17a}\end{align}
A useful consequence is the equation for the quantity $fv$, \textbf{{*}{*}{*}here
is a mistake!} \textbf{this Eq.~(\ref{eq:fv equ 17a}) does not follow. So
all the following calculations are probably useless.}\begin{equation}
\frac{d}{d\psi}\ln\left(fv\right)=-1-\frac{Q_{2}}{v^{n}}\left(\ln K\right)_{,\psi}.\label{eq:fv equ 17a}\end{equation}


We are looking for solutions with $v\rightarrow0$ and $f\rightarrow+\infty$
as $\psi\rightarrow\infty$. A necessary condition for the existence of such
solutions is found by taking the limit of Eq.~(\ref{eq:v equ 17a}) as $\phi\rightarrow\infty$,\begin{equation}
\lim_{\phi\rightarrow\infty}\frac{d\ln K}{d\ln\phi}\frac{1}{v^{n-1}}=0\quad\Rightarrow\quad\lim_{\phi\rightarrow\infty}\frac{d\ln K}{d\ln\phi}=0.\label{eq:K cond 17a}\end{equation}
It means that $K(\phi)$ grows or decays at $\phi\rightarrow\infty$ slower
than any power of $\phi$. 

Considering now the limit of Eq.~(\ref{eq:f equ 17a}) as $\psi\rightarrow\infty$,
we notice that the left-hand side of Eq.~(\ref{eq:f equ 17a}) must be positive
due to the growth of $f$, and thus the quantity $fv$ must remain between 0
and 1 as $\phi\rightarrow\infty$. Assuming that the general solution $\left\{ f(\psi),v(\psi)\right\} $
has the properties $v\rightarrow0$ and $f\rightarrow\infty$, there are only
two possibilities: either for every solution (except perhaps finitely many)\begin{equation}
\lim_{\psi\rightarrow\infty}fv\equiv p_{0},\quad0<p_{0}\leq1,\label{eq:limit fv is p0}\end{equation}
where the constant $p_{0}$ may or may not depend on the particular solution;
or the limit $p_{0}$ is zero for every solution (again, except perhaps for
finitely many). We will now consider these two cases. The possibility remains
that finitely many exceptional solutions exist for which $p_{0}$ is different,
but these solutions can be disregarded for the purposes of stability analysis.

First, we assume that Eq.~(\ref{eq:limit fv is p0}) holds for \emph{some}
solution $\left\{ f,v\right\} $ such that $f\rightarrow\infty$ and $v\rightarrow0$.
Then it follows from Eq.~(\ref{eq:fv equ 17a}) that\begin{equation}
\lim_{\psi\rightarrow\infty}\frac{Q_{2}}{v^{n}}\left(\ln K\right)_{,\psi}=-1.\label{eq:limit 17b}\end{equation}
So the only admissible $K(\phi)$ are such that\begin{equation}
\frac{d\ln K(\phi)}{d\ln\phi}<0;\end{equation}
in particular, it is necessary to have $dK(\phi)/d\phi<0$ at large $\phi$.
Since the asymptotic behavior of $K(\phi)$ at $\phi\rightarrow\infty$ is fixed
by the Lagrangian, it follows that every admissible solution $v$ must have
the following asymptotic behavior, \begin{equation}
v(\psi)=\left[-Q_{2}\left(\ln K\right)_{,\psi}\right]^{\frac{1}{n}}\left[1+A(\psi)\right],\quad\lim_{\psi\rightarrow\infty}A(\psi)=0.\end{equation}
The corresponding ansatz for $f(\phi)$ is\begin{equation}
f(\psi)=\frac{p_{0}}{v(\psi)}\left[1+B(\psi)\right],\quad\lim_{\psi\rightarrow\infty}B(\psi)=0.\end{equation}
Here $A(\psi)$ and $B(\psi)$ are new unknown funtions. Substituting these
expressions for $f$ and $v$ into Eqs.~(\ref{eq:v equ 17a}) and (\ref{eq:fv equ 17a}),
we find, to the leading order in $A$ and $B$,\begin{align}
\frac{dA}{d\psi} & =-\frac{1}{n}\frac{\left(\ln K\right)_{,\psi\psi}}{\left(\ln K\right)_{,\psi}}+\left(1-nA\right)-\frac{1-B}{p_{0}},\label{eq:A equ 17b}\\
\frac{dB}{d\psi} & =-A.\label{eq:B equ 17b}\end{align}
A necessary condition for the existence of solutions with $A\rightarrow0$,
$B\rightarrow0$ is\begin{equation}
\lim_{\psi\rightarrow\infty}\frac{\left(\ln K\right)_{,\psi\psi}}{\left(\ln K\right)_{,\psi}}=n\left(1-\frac{1}{p_{0}}\right)\leq0.\label{eq:p0 def}\end{equation}
This determines the value of $p_{0}$. For $0<p_{0}<1$, the function $K(\phi)$
must have the asymptotic form\begin{equation}
K(\phi)\approx K_{0}\left(1+K_{1}\phi^{-s}\right),\quad\phi\rightarrow\infty,\; K_{1}>0,\; s>0,\label{eq:K form 17b}\end{equation}
for which the value of $p_{0}$ is\begin{equation}
p_{0}=\frac{n}{n+s}.\end{equation}
However, $K(\phi)$ cannot tend to a constant faster than an inverse power of
$\phi$; for instance, $K(\phi)\propto1+K_{1}e^{-s\phi}$ are not admissible
since the limit in Eq.~(\ref{eq:p0 def}) is infinite. If $K(\phi)$ tends
to a constant (or to zero) slower than any power of $\phi$, the corresponding
value of $p_{0}$ is $p_{0}=1$.

Assuming that $p_{0}$ satisfies Eq.~(\ref{eq:p0 def}) and $0<p_{0}\leq1$,
we now need to analyze the stability of the general solution of Eqs.~(\ref{eq:A equ 17b})--(\ref{eq:B equ 17b}).
This analysis proceeds in the standard way; the stability conditions are $n>0$,
$p_{0}>0$. Thus the solution is asymptotically stable when the condition~(\ref{eq:K cond 17a})
holds, $dK/d\phi<0$ at large $\phi$, and $0<p_{0}\leq1$, where $p_{0}$ is
determined from Eq.~(\ref{eq:p0 def}). This is a transient attractor since
$w_{\phi}\rightarrow-1$ and the energy density of $k$-essence will eventually
start to dominate. This attractor exists, in particular, when $K(\phi)$ is
of the form~(\ref{eq:K form 17b}), but is not limited to such $K(\phi)$.

It remains to consider the case $\lim_{\psi\rightarrow\infty}fv=0$. This case
may be realized only if $K(\phi)$ tends to a constant at $\phi\rightarrow\infty$
faster than any power of $\phi$; then the left-hand side of Eq.~(\ref{eq:p0 def})
tends to a negative infinity. We now consider the possible values of the limit~(\ref{eq:limit 17b}),
which is now not necessarily equal to $-1$. Evaluating the limit of Eq.~(\ref{eq:fv equ 17a})
at $\psi\rightarrow\infty$ and taking into account the assumption $fv\rightarrow0$,
we find that the function\begin{equation}
q(\psi)\equiv\frac{Q_{2}}{v^{n}}\left(\ln K\right)_{,\psi}\end{equation}
cannot stay below $-1$ at large $\psi$. Thus we have two possibilities: either
$q(\psi)$ tends to a finite limit, \begin{equation}
\lim_{\psi\rightarrow\infty}q(\psi)\equiv q_{0}\geq-1,\end{equation}
or $q(\psi)\rightarrow+\infty$. To investigate the behavior of $q(\psi)$,
we use the equation\begin{equation}
\frac{d\ln q}{d\psi}=nq+\frac{n}{fv}-N(\psi),\quad N(\psi)\equiv-\frac{\left(\ln K\right)_{,\psi\psi}}{\left(\ln K\right)_{,\psi}},\label{eq:q equ 17c}\end{equation}
which follows straightforwardly from Eq.~(\ref{eq:v equ 17a}) and definition
of $q(\psi)$. The function $N(\psi)$ tends to a positive infinity at $\psi\rightarrow\infty$
because, by assumption, the left-hand side of Eq.~(\ref{eq:p0 def}) tends
to a negative infinity. We also rewrite Eq.~(\ref{eq:fv equ 17a}) as\begin{equation}
\frac{d}{d\psi}\ln\left(\frac{1}{fv}\right)=q(\psi)+1.\label{eq:fv equ 17c}\end{equation}


First, we treat the case where \begin{equation}
\lim_{\psi\rightarrow\infty}q(\psi)=q_{0},\end{equation}
 where $q_{0}\geq-1$ is a finite constant. Let us temporarily assume that $q_{0}\neq0$,
and postpone the consideration of the case $q_{0}=0$. Then we examine Eq.~(\ref{eq:q equ 17c})
at large $\psi$ and obtain the asymptotic relationship\begin{equation}
\lim_{\psi\rightarrow\infty}\left[nq+\frac{n}{fv}-N(\psi)\right]=0.\end{equation}
Since the function $N(\psi)$ is fixed by the Lagrangian, the possible solutions
$\left\{ f,v\right\} $ are constrained to the form\begin{equation}
fv=\frac{n}{N(\psi)-nq_{0}+B(\psi)},\quad\lim_{\psi\rightarrow\infty}B(\psi)=0.\end{equation}
Substituting this ansatz into Eq.~(\ref{eq:fv equ 17c}) and taking the limit
at $\psi\rightarrow\infty$, we find\begin{equation}
\lim_{\psi\rightarrow\infty}\frac{d}{d\psi}\ln N(\psi)=q_{0}+1.\end{equation}
This determines the admissible value of $q_{0}$ for a given $N(\psi)$; for
instance, $q_{0}=-1$ if $N(\psi)$ grows slower than exponentially in $\psi$,
while faster-than-exponential growth is not admissible in the present case.
Also, growth as $N(\psi)\propto e^{\psi}$ is not allowed, since that would
correspond to $q_{0}=0$. Assuming that $N(\psi)$ satisfies these restrictions,
we use the ansatz\begin{equation}
q(\psi)=q_{0}+A(\psi),\quad\lim_{\psi\rightarrow\infty}A(\psi)=0,\end{equation}
and derive the equations for the functions $A(\psi)$, $B(\psi)$ in the leading
order:\begin{align}
\frac{dA}{d\psi} & =nq_{0}A+q_{0}B,\\
\frac{dB}{d\psi} & =-\left(1+q_{0}\right)\left[nq_{0}-B\right]+NA+\left[q_{0}+1-\left(\ln N\right)_{,\psi}\right]N.\end{align}
This is an inhomogeneous, linear system of equations with time-dependent coefficients.
We need the general solution $\{ A(\psi),B(\psi)\}$ of this system to be stable,
i.e.~such that $A\rightarrow0$ and $B\rightarrow0$ at $\psi\rightarrow\infty$.
A necessary condition for the stability is the stability of the homogeneous
system,\begin{align}
\frac{dA}{d\psi} & =nq_{0}A+q_{0}B,\\
\frac{dB}{d\psi} & =\left(1+q_{0}\right)B+NA.\end{align}
We note that all the coefficients in the above system are positive, with the
exception of $1+q_{0}$ which may be positive or vanish. It follows that the
solutions (with positive initial values $A,B$) are growing at least exponentially
quickly in $\psi$. Hence, stability of the general solution of this system
is impossible.

Similar considerations preclude the stability of the general solution when \begin{equation}
\lim_{\psi\rightarrow\infty}q=0,\quad\lim_{\psi\rightarrow\infty}\left(\ln q\right)_{,\psi}=q_{1},\end{equation}
 where $q_{1}$ is a finite nonpositive constant (the case $q_{1}=0$ is included).
The general solution must have the asymptotic behavior\begin{equation}
fv=\frac{n}{N(\psi)-q_{1}+B(\psi)},\quad\lim_{\psi\rightarrow\infty}B(\psi)=0.\end{equation}
Substituting this ansatz into Eqs.~(\ref{eq:q equ 17c}) and (\ref{eq:fv equ 17c}),
we obtain in the leading order\begin{align}
\frac{dq}{d\psi} & =-q_{1}q+nq^{2}+Bq,\\
\frac{dB}{d\psi} & =B+qN+N-N'-q_{1}.\end{align}
The absence of stability in the general solution becomes apparent if we consider
the possible particular solution where $qN$ is much smaller than $B$, so these
equations can be simplified to\begin{align}
\frac{dq}{d\psi} & =-q_{1}q+Bq,\\
\frac{dB}{d\psi} & =B+N-N'-q_{1}.\end{align}
It is clear that the solution $B(\psi)$ of the homogeneous system grows exponentially
(regardless of whether $q_{1}=0$). Therefore, stability is absent in this case. 

The remaining possibility is\begin{equation}
\lim_{\psi\rightarrow\infty}q=0,\quad\lim_{\psi\rightarrow\infty}\left(\ln q\right)_{,\psi}=-\infty.\end{equation}
In other words, $q$ tends to zero faster than any exponential of the form $\exp\left(-C_{0}\psi\right)$.
In this case, the condition that the original variable $v(\phi)\rightarrow0$
is equivalent to\begin{equation}
\lim_{\psi\rightarrow\infty}\frac{\left(\ln K\right)_{,\psi}}{q(\psi)}=0.\label{eq:condition v 17c}\end{equation}
We find from Eq.~(\ref{eq:fv equ 17c}) that $1/\left(fv\right)$ grows as\begin{equation}
\frac{1}{fv}=C_{1}e^{\psi}\left[1+B(\psi)\right],\quad\lim_{\psi\rightarrow\infty}B(\psi)=0,\end{equation}
where $C_{1}$ is an arbitrary constant. It then follows from Eq.~(\ref{eq:q equ 17c})
that $N(\psi)$ must grow at least as fast with $\psi$. Assuming that this
is the case, we may rewrite Eqs.~(\ref{eq:q equ 17c}) and (\ref{eq:fv equ 17c})
as\begin{align}
\frac{d\ln q}{d\psi} & =nq+nC_{1}e^{\psi}\left[1+B\right]-N(\psi),\\
\frac{dB}{d\psi} & =q(\psi).\end{align}
Using the definition of $N(\psi)$ in Eq.~(\ref{eq:q equ 17c}), we find an
approximate general solution for very small $B$ and $q$, with arbitrary constants
$C_{0}$ and $C_{1}$, as\begin{align}
B(\psi) & \approx-\int_{\psi}^{\infty}q(\psi)d\psi,\\
q(\psi) & \approx\exp\left[C_{0}+nC_{1}e^{\psi}\right]\left(\ln K\right)_{,\psi}.\end{align}
The integral $\int q(\psi)d\psi$ converges due to a fast decay of $q(\psi)$;
the constant of integration for $B(\psi)$ is absorbed in the definition of
$C_{1}$. It is clear that the condition~(\ref{eq:condition v 17c}) holds
for this solution. Therefore, this solution represents a transient attractor.
This attractor is present when $K(\phi)$ tends to a constant at $\phi\rightarrow\infty$
exponentially fast or faster.

In the second case under consideration, it is assumed that $q(\psi)\rightarrow\infty$.
It then follows from Eq.~(\ref{eq:fv equ 17c}) that the function $-\ln\left(fv\right)$
grows faster than linearly in $\psi$ at $\psi\rightarrow\infty$. Moreover,
the function $1/\left(fv\right)$ grows much faster than $q(\psi)$, while both
tend to infinity: To show that \begin{equation}
\lim_{\psi\rightarrow\infty}\frac{1}{fvq}=\infty,\end{equation}
it suffices to compute the derivative using Eq.~(\ref{eq:fv equ 17c}) and
assuming that $q\rightarrow\infty$,\begin{align}
\frac{d}{d\psi}\left(\frac{1}{fvq}\right) & =\frac{1}{fvq}\left(q+1\right)-\frac{1}{fvq^{2}}\frac{dq}{d\psi}\nonumber \\
 & =\frac{1}{fv}\left(1+\frac{1}{q}-\frac{d}{d\psi}\frac{1}{q}\right)\rightarrow\infty.\end{align}
 Therefore, the term $nq$ in Eq.~(\ref{eq:q equ 17c}) is always negligible
compared with the term $n/\left(fv\right)$. Since the right-hand side of Eq.~(\ref{eq:q equ 17c})
must be positive at large $\psi$, we find that $1/(fv)$ must grow at least
as fast as $N(\psi)$. Hence, we are lead to considering two possibilities:
either $n/(fv)\geq N(\psi)$ for all sufficiently large $\psi$, or \begin{equation}
\frac{n}{fv}<N(\psi),\quad\lim_{\psi\rightarrow\infty}\frac{n}{fvN}=1.\label{eq:cond 17d}\end{equation}
If $n/(fv)\geq N(\psi)$, we find from Eq.~(\ref{eq:q equ 17c}) that \begin{equation}
\frac{d\ln q}{d\psi}\geq nq.\end{equation}
It follows that \begin{equation}
q(\phi)\geq\frac{1}{C_{2}-n\psi},\end{equation}
where $C_{2}$ is an unknown integration constant. For any $C_{2}$, $q(\psi)$
reaches infinity at a \emph{finite} value of $\psi$; this is clearly not compatible
with the assumption that arbitrarily large values of $\psi$ are reached at
sufficiently late times. Therefore this case does not yield any attractors of
the assumed type.

It remains to consider the possibility that Eq.~(\ref{eq:cond 17d}) holds.
In that case, we may use the ansatz\begin{equation}
\frac{n}{fv}=N(\psi)\left[1+B(\psi)\right],\quad\lim_{\psi\rightarrow\infty}B(\psi)=0,\end{equation}
and compute $q(\psi)$ from Eq.~(\ref{eq:fv equ 17c}) to the leading order
as\begin{equation}
q(\psi)=\frac{d}{d\psi}\ln\left(\frac{1}{fv}\right)-1=\left(\ln N\right)_{,\psi}+B_{,\psi}-1.\end{equation}
Since by assumption $B\rightarrow0$, it is necessary to have $\left(\ln N\right)_{,\psi}\rightarrow\infty$
at $\psi\rightarrow\infty$. Thus we may replace $\left(\ln N\right)_{,\psi}-1$
by $\left(\ln N\right)_{,\psi}$ and write\begin{equation}
q(\psi)\approx\left(\ln N\right)_{,\psi}+B_{,\psi}.\end{equation}
 We now substitute the expression for $q(\psi)$ above into Eq.~(\ref{eq:q equ 17c})
and obtain, to the leading order,\begin{align}
B_{,\psi\psi} & =-\left(\ln N\right)_{,\psi\psi}+\left[\left(\ln N\right)_{,\psi}\right]^{2}n\nonumber \\
 & +2\left(\ln N\right)_{,\psi}B_{,\psi}n+N_{,\psi}B.\end{align}
This is an inhomogeneous linear equation for $B(\psi)$; we need its general
solution $B(\psi)$ to tend to zero at $\psi\rightarrow\infty$. However, the
coefficients in the right-hand side of this equation grow to infinity, so the
corresponding homogeneous equation always has growing solutions. Therefore,
an asymptotically stable solution does not exist.


\subsection{Slow motion ($v_{0}=0$), marginal cases}

In this section we consider the case $v_{0}=0$, $Q(0)=0$, and assume the expansion~(\ref{eq:Q expansion 3a}).
The decompositions~(\ref{eq:wk expansion 3a})--(\ref{eq:cs expansion 3a})
apply; the solution will be a transient attractor if the asymptotic value of
the equation-of-state parameter, $w_{\phi}(0)=\frac{1}{n-1}$, is not above
the value $w_{m}$. 

We rewrite Eqs.~(\ref{eq:v equ 15})--(\ref{eq:h equ 15}) to leading order
as\begin{align}
\frac{dv}{d\phi} & =-\frac{v}{n}\frac{K'}{K}-\frac{1}{n-1}h^{-1},\label{eq:v equ 18}\\
\frac{dh}{d\phi} & =\frac{1+w_{m}}{2}v^{-1}.\label{eq:h equ 18}\end{align}
A linear combination of these equations gives\begin{equation}
\frac{d\ln v}{d\phi}+\frac{2}{\left(n-1\right)\left(1+w_{m}\right)}\frac{d\ln h}{d\phi}+\frac{1}{n}\frac{d\ln K}{d\phi}=0,\end{equation}
which is integrated to\begin{equation}
vh^{1/\alpha}K^{1/n}=\textrm{const},\quad\alpha\equiv\frac{\left(n-1\right)\left(1+w_{m}\right)}{2}.\label{eq:cons law 18}\end{equation}
Since by assumption $w_{m}\geq\frac{1}{n-1}$, the constant $\alpha$ satisfies
$\alpha\geq n/2$, and in particular $\alpha\geq1$ because $n\geq2$. We then
express $h(\phi)$ through $v(\phi)$ using Eq.~(\ref{eq:cons law 18}), \begin{equation}
h^{-1}=\left(n-1\right)C_{0}v^{\alpha}K^{\alpha/n},\end{equation}
where $(n-1)C_{0}>0$ is an arbitrary integration constant, and substitute into
Eq.~(\ref{eq:v equ 18}) to obtain \begin{equation}
\frac{dv}{d\phi}=-\frac{v}{n}\frac{K'}{K}-C_{0}v^{\alpha}K^{\alpha/n}.\label{eq:v equ 18a}\end{equation}
This equation can be transformed into\begin{equation}
\frac{d}{d\phi}\left[vK^{1/n}\right]=-C_{0}\left[vK^{1/n}\right]^{\alpha}K^{1/n},\end{equation}
and integrated,\begin{equation}
v(\phi)=\begin{cases}
K^{-1/n}\exp\left[C_{1}-C_{0}\int^{\phi}K^{1/n}d\phi\right], & \alpha=1,\\
K^{-1/n}\left[C_{1}+C_{0}\left(\alpha-1\right)\int^{\phi}K^{1/n}d\phi\right]^{-1/(\alpha-1)}, & \alpha>1.\end{cases}\label{eq:v sol 18}\end{equation}
 We note that the case $\alpha=1$ is possible only when $n=2$ and $w_{m}=1=w_{\phi}(0)$.

We require that the general solution $v(\phi)$ tend to zero at $\phi\rightarrow\infty$,
and that the energy density of $k$-essence eventually dominates over that of
matter. The energy dominance is assured if $w_{m}>w_{\phi}(0)=\frac{1}{n-1}$,
but the borderline case $w_{m}=\frac{1}{n-1}$ (corresponding to $\alpha=n/2$)
needs to be investigated separately. In that case, we may rewrite the ratio
$\varepsilon_{\phi}/\varepsilon_{m}$ as\begin{equation}
\frac{\sqrt{\varepsilon_{\phi}}}{3\kappa\sqrt{\varepsilon_{m}}}=\sqrt{\left(n-1\right)Q_{1}}hv^{n/2}=\frac{\sqrt{Q_{1}}}{\sqrt{n-1}C_{0}}K^{-1/2},\end{equation}
where we have used Eqs.~(\ref{eq:epsilon expansion 3a}), (\ref{eq:h def 15}),
and (\ref{eq:cons law 18}) with $\alpha=n/2$. Therefore, in this borderline
case the energy density of $k$-essence will eventually dominate only if $K(\phi)$
decays at $\phi\rightarrow\infty$.

It remains to investigate the stability of the general solution $v(\phi)$ given
by Eq.~(\ref{eq:v sol 18}). We use arguments similar to those used in the
analysis of Eqs.~(\ref{eq:cond F 12 a})--(\ref{eq:cond F 12 b}). If the integral
$\int^{\infty}K^{1/n}(\phi)d\phi$ converges (which is possible only when $K(\phi)\rightarrow0$
at $\phi\rightarrow\infty$), the general solution $v(\phi)$ tends to infinity.
Therefore, the divergence of the integral $\int^{\infty}K^{1/n}(\phi)d\phi$
is a necessary condition. It is clear that the general solution $v(\phi)$ will
tend to zero if $K(\phi)$ grows sufficiently quickly at $\phi\rightarrow\infty$;
the slower the growth of $K(\phi)$, the slower will $v(\phi)$ tend to zero.
Therefore, we determine the borderline class of functions $K(\phi)$ for which
$v(\phi)$ tends to a nonzero constant. Such $K(\phi)$ can be easily determined
directly from Eq.~(\ref{eq:v equ 18a}) by substituting $v=v_{0}$, $v_{0}\neq0$
as the solution at large $\phi$. The resulting $K(\phi)$ have the large-$\phi$
behavior of the form \begin{equation}
K(\phi)\propto\phi^{-n/\alpha},\quad\alpha\geq1.\end{equation}
 Thus the admissible $K(\phi)$ must be such that\begin{equation}
\lim_{\phi\rightarrow\infty}\phi^{n/\alpha}K(\phi)=\infty,\quad\alpha\geq1.\end{equation}
 The divergence of the integral $\int^{\infty}K^{1/n}(\phi)d\phi$ is then assured,
although these $K(\phi)$ tend to zero at $\phi\rightarrow\infty$. The energy
domination condition is satisfied also in the borderline case $\alpha=n/2$,
as long as $K(\phi)\rightarrow0$ at $\phi\rightarrow\infty$. Therefore, these
solutions represent stable transient attractors under the cited conditions.


\section{Very slow motion}

Throughout the analysis in the previous sections, we have assumed that the $k$-essence
field $\phi$ can reach arbitrarily large values in the course of the attractor
solution. An alternative possibility is that the velocity $v\equiv\dot{\phi}$
goes to zero so quickly that $\phi(t)$ tends to a finite limit at $t\rightarrow\infty$.
In this section we investigate the possibility of stable attractor solutions
of this type.

It is useful to consider the cases $Q(0)\neq0$ and $Q(0)=0$ separately.


\subsection{Very slow motion, main case ($Q(0)\neq0$)}

In this case we may use the expansions~(\ref{eq:Q expansion 3})--(\ref{eq:cs expansion 3})
and rewrite the equations of motion~(\ref{eq:v equ clever})--(\ref{eq:R EOM})
to leading order in $v$ as\begin{align}
\ddot{\phi}=v\frac{dv}{d\phi} & =-\frac{1}{n-1}\left[\frac{\left(\ln K\right)_{,\phi}Q_{0}}{nQ_{1}v^{n-2}}+3\kappa v\sqrt{\frac{K(\phi)Q_{0}}{1-R}}\right],\label{eq:v equ 19}\\
\dot{R}=v\frac{dR}{d\phi} & =-3\kappa R\sqrt{1-R}\sqrt{K(\phi)Q_{0}}\left(w_{m}+1\right).\label{eq:R equ 19}\end{align}
We are looking for solutions that tend to constant values, $\phi\rightarrow\phi_{0}$
and $R\rightarrow R_{0}$, as $t\rightarrow\infty$. Thus we have $\ddot{\phi}\rightarrow0$
and $\dot{R}\rightarrow0$ at $\phi\rightarrow\phi_{0}$. Since the right-hand
side of Eq.~(\ref{eq:R equ 19}) is never positive, $R(t)$ cannot grow and
hence the possibility $R_{0}=1$ (asymptotically negligible $k$-essence energy
density) is excluded. Evaluating the limit of Eqs.~(\ref{eq:v equ 19})--(\ref{eq:R equ 19})
at $\phi\rightarrow\phi_{0}$ and using the assumptions $n\geq2$ and $v\rightarrow0$,
we then obtain the necessary conditions\begin{align}
\lim_{\phi\rightarrow\phi_{0}}\left(\ln K\right)_{,\phi} & =\lim_{\phi\rightarrow\phi_{0}}\frac{K'(\phi)}{K(\phi)}=0,\\
\lim_{\phi\rightarrow\phi_{0}}R\sqrt{K} & =R_{0}K(\phi_{0})=0.\end{align}
It follows that $K(\phi_{0})\neq0$, $K'(\phi_{0})=0$, and $R_{0}=0$. We may
expand $K(\phi)$ near $\phi=\phi_{0}$ as\begin{equation}
K(\phi)\approx K_{0}\left[1+K_{1}\left(\phi-\phi_{0}\right)^{m}\right],\quad m\geq2,\quad K_{0}\neq0,\quad K_{1}\neq0.\end{equation}
 Hence, near $\phi=\phi_{0}$ we have the equations\begin{align}
\ddot{\phi} & =-\frac{3\kappa\sqrt{K(\phi_{0})Q_{0}}}{n-1}\dot{\phi}-\frac{mQ_{0}K_{1}}{n\left(n-1\right)Q_{1}}\frac{\left(\phi-\phi_{0}\right)^{m-1}}{\dot{\phi}^{n-2}},\label{eq:v equ 19a}\\
\frac{d}{dt}R & =-3\kappa R\sqrt{K(\phi_{0})Q_{0}}\left(w_{m}+1\right).\end{align}
It is clear that the general solution $R(t)$ tends to zero at $t\rightarrow\infty$
when $w_{m}>-1$. It remains to verify that the general solution $\phi(t)\rightarrow\phi_{0}$
as $t\rightarrow\infty$. \textbf{{*}{*}{*}}


\subsection{Very slow motion, marginal cases ($Q(0)=0$)}

We use the expansions~(\ref{eq:Q expansion 3a})--(\ref{eq:cs expansion 3a})
and rewrite the equations of motion~(\ref{eq:v equ clever})--(\ref{eq:R EOM})
to leading order in $v$ as\begin{align}
\ddot{\phi}=v\frac{dv}{d\phi} & =-\frac{1}{n}v^{2}\left(\ln K\right)_{,\phi}-3\kappa\frac{1}{\sqrt{n-1}}v^{1+\frac{n}{2}}\sqrt{\frac{K(\phi)Q_{1}}{1-R}},\\
\dot{R}=v\frac{dR}{d\phi} & =-3\kappa v^{n/2}R\sqrt{1-R}\sqrt{K(\phi)\left(n-1\right)Q_{1}}\left(w_{m}-w_{\phi}(v)\right).\end{align}
The asymptotic value of $w_{\phi}(v)$ is $\frac{1}{n-1}$. If $w_{m}\neq\frac{1}{n-1}$,
the second equation simplifies to\begin{equation}
\dot{R}=-3\kappa v^{n/2}R\sqrt{1-R}\sqrt{K(\phi)\left(n-1\right)Q_{1}}\left(w_{m}-\frac{1}{n-1}\right).\end{equation}
If $w_{m}=\frac{1}{n-1}$, we assume the expansion~(\ref{eq:Q expansion v2}),
and the equation for $R(t)$ becomes\begin{equation}
\dot{R}=-3\kappa v^{n/2+p}R\sqrt{1-R}\frac{\sqrt{K(\phi)Q_{1}}pQ_{2}}{\left(n-1\right)^{3/2}Q_{1}}.\end{equation}
\textbf{{*}{*}{*}}


\subsection{Very slow motion, transient attractors, main case ($Q(0)\neq0$)}

We also analyze the possibility of transient attractors with very slow motion.
First we consider the case $Q(0)\neq0$, where the expansions~(\ref{eq:Q expansion 3})--(\ref{eq:cs expansion 3})
apply. As before, we define $h(\phi)$ by Eq.~(\ref{eq:h def 15}) and rewrite
the equations of motion~(\ref{eq:v equ 15})--(\ref{eq:h equ 15}) as\begin{align}
\ddot{\phi}=v\frac{dv}{d\phi} & =-\frac{Q_{0}}{n\left(n-1\right)Q_{1}}v^{2-n}\frac{K'}{K}-\frac{v}{\left(n-1\right)h},\\
\dot{h}=v\frac{dh}{dv} & =\frac{1+w_{m}}{2}.\end{align}
The equation for $h(t)$ can be integrated immediately,\begin{equation}
h(t)=h_{0}+\frac{1+w_{m}}{2}t.\end{equation}



\subsection{Very slow motion, transient attractors, marginal cases ($Q(0)=0$)}

Now we consider the case $Q(0)=0$, where the expansions~(\ref{eq:Q expansion 3a})--(\ref{eq:cs expansion 3a})
apply. Using these expansions, we rewrite the equations of motion~(\ref{eq:v equ 15})--(\ref{eq:h equ 15})
as\begin{align}
\ddot{\phi}=v\frac{dv}{d\phi} & =-\frac{1}{n}v^{2}\frac{K'}{K}-\frac{v}{\left(n-1\right)h},\\
\dot{h}=v\frac{dh}{dv} & =\frac{1+w_{m}}{2}.\end{align}
The equation for $h(t)$ can be integrated immediately,\begin{equation}
h(t)=h_{0}+\frac{1+w_{m}}{2}t.\end{equation}


